Semi-Supervised Clustering with Neural Networks

Clustering using neural networks has recently demonstrated promising performance in machine learning and computer vision applications. However, the performance of current approaches is limited either by unsupervised learning or their dependence on large set of labeled data samples. In this paper, we propose ClusterNet that uses pairwise semantic constraints from very few labeled data samples (<5% of total data) and exploits the abundant unlabeled data to drive the clustering approach. We define a new loss function that uses pairwise semantic similarity between objects combined with constrained k-means clustering to efficiently utilize both labeled and unlabeled data in the same framework. The proposed network uses convolution autoencoder to learn a latent representation that groups data into k specified clusters, while also learning the cluster centers simultaneously. We evaluate and compare the performance of ClusterNet on several datasets and state of the art deep clustering approaches.

==> Sections/frgc_acc.tex <==
\begin{table*}[h]
{\small 
	\centering
		\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Labeled Data (\%)  & {ClusterNet} & NNClustering& JULE & DEPICT & CPAC \\ \hline
    2    & &&& \\ \cline{1-3} 
    5    & $\pm$ 0.027& &&& \\ \cline{1-3}
    10    &0.955$\pm$ &&& \\ \cline{1-3}
    50    & $\pm$ &&& \\\hline  	
	\end{tabular}
	\caption{FRGC Dataset NMI Results}
	\label{tab: frgc_nmi}
}
\end{table*}

==> Sections/frgc_oos.tex <==
\begin{table}[h]
{\small 
	\centering
		\begin{tabular}{|c|p{1.8cm}|p{1.9cm}|}
		\hline
Labeled Data (\%)  & \multicolumn{2}{c|}{ClusterNet}\\\cline{2-3}
 & NMI & ACC (\%)\\\hline
    2    & 0.681$\pm$0.075 &60.16$\pm$11.86\\ \hline
    5    & 0.885$\pm$ 0.027& 87.86  $\pm$ 4.32\\ \hline
    10    &0.955$\pm$ 0.011&96.07 $\pm$1.24\\ \hline
    50    &0.974 $\pm$ 0.012 & 97.73 $\pm$ 0.84\\\hline  	
	\end{tabular}
	\caption{FRGC Dataset Out of Sample Results}
	\label{tab: frgc_oos}
}
\end{table}

==> Sections/table1.tex <==
\begin{table}[h]
{\small 
	\centering
		\begin{tabular}{|c|c|c|c|c|}
		\hline
		Labeled Data   & \multicolumn{3}{c|}{ACC} \\ \cline{2-4}
      &  SWWAE  & DEPICT  & ClusterNet   \\\hline
%       60  & 79.4 & &\textbf{88.15}\\\hline
      100  & 8.71 $\pm$0.34&2.65 $\pm$0.35 & -- \\\hline
%       600  &95.1&&\textbf{98.04}\\ \hline
      1000 &2.83 $\pm$0.10& 2.10 $\pm$0.11& \textbf{2.02 $\pm$ 0.21} \\\hline
      3000 &2.10 $\pm$ 0.22 &1.91 $\pm$ 0.06& \textbf{1.65 $\pm$ 0.10} \\\hline
%       6000  &98.8  &  &   \\\hline
 	
	\end{tabular}
    \vspace{0.1cm}
	\caption{Comparison of SSWAE \cite{Zhao_2015} and DEPICT \cite{Dizaji_ICCV2017} classification models (trained with cross entropy loss after trained for clustering loss) with \cnet clustering model for classification performance. For \cnet, we use the explicitly computed cluster centers to identify the labels of unseen data samples. All the results are reported on \textit{MNIST-test}}
	\label{tab: comp}
}
\end{table}

==> Sections/table_clustering.tex <==
\begin{table*}[h]
{\small 
	\centering
		\begin{tabular}{|c|c|p{1.6cm}|c|}
		\hline
		Labeled Data (\%)  & Unlabeled Data& Clustering & Classification\\ \hline
  	
	\end{tabular}
	\caption{}
	\label{tab:}
}
\end{table*}
